Characterizing Lagrangian particle dynamics in decaying HIT using proper orthogonal decomposition

The particle proper orthogonal decomposition (PPOD) is demonstrated on cases of particle flows in decaying homogeneous isotropic turbulence. Data is generated through one-way coupled simulations, where particle positions and velocities are integrated forward in time in a Lagrangian manner. The PPOD offers a direct way of extracting statistical information on the dispersed (discrete) phase of multiphase flows without any underlying assumptions. Furthermore, the method gives the possibility of modal analysis of fluid-particle interactions in multiphase flows, an example of which is provided in this work. The results demonstrate a proof of concept of the PPOD, and potential of applicability. Additionally, the results suggest that the PPOD-modes can be used for approximating particle trajectories/velocities within turbulent flows.

==> Sections/FurtherWork.tex <==
\iffalse
- Test on more physical systems
    • Two-way coupled, four-way coupled -- OK
    • Non-HIT -- OK
- Test on larger temporal domains (PPOD efficacy might become worse).
- More density analysis. Different particle sizes.
- Test using more particle-driving forces.  --OK
- Test on more particles pr. Realization
    • Consider what the particle initial configuration should be. 
- Test with more realizations.
- Discuss the applicability of PPOD on the Navier-Stokes equation (Is there a reference from Azur here??)

Further work
- Not only drag force
\fi

The analysis of \autoref{sec:Results} provides a proof of concept of the PPOD as a method for extracting statistical information on the dispersed phase of multiphase flows. It shows potential in modal approximation of particle dynamics and in statistical analysis of fluid-particle interactions. However, the method has yet to be tested on a variety of configurations. These configurations include (more) physical systems such as two-way or four-way coupled particle-laden flows, or turbulent flows that are non-HIT. Such studies may show that PPOD is ineffective when the analyzed system becomes more complex, however they may also show that PPOD is a powerful tool for such an analysis. \\
In this work realizations consisted of particles that were accelerated according to drag force only. Iteratively adding more forces to this acceleration and applying PPOD in between may yield insights on how each force affects the trajectory of a particle. A modification of equation \eqref{eq:NormedDiff} can be used for such a study, where a comparison of each type of realization can be carried out, to reveal which modes the added force has influenced. Since each mode comes with a corresponding eigenvalue representing particle kinetic energy, the contribution of the added force is easily quantifiable. \\
PPOD has yet to be tested on larger cases. In this study we considered a maximum of $N_p=20$ particles pr. realization, and $N_t = 1001$ temporal samples. Increasing $N_p$ may result in computational infeasibility due to memory issues. Increasing $N_t$ may result in a lower convergence rate, since each mode needs to "cover" a larger temporal domain. 


\iffalse
As already mentioned these configurations include physical systems, such as two-way or four-way coupled particle-laden flows. Turbulent flows that are non-HIT are also cases where PPOD should be tested. Furthermore, a more extensive study on how particle parameters such as density, volume and shape affect the resulting PPOD modes may prove insightful. \\
This study was performed on cases of at most $N_p = 20$ particles pr. realization. Additionally the particles were only affected by drag force. These are two are parameters that also need to be analyzed more thoroughly. For instance, how well does the PPOD perform when ten thousand particles pr. realization are considered? And when these particles are spread out in the whole domain? Perhaps such a study will reveal that the method in question is more useful in decomposing the velocity of a small cluster of particles with low separation between them, than it is at decomposing the velocity of the all particles of the dispersed phase simultaneously. \\
A modal decomposition of various particle simulations, where different forces are used to accelerate the particles may yield insights into 
\fi
